Zero-shot Cross-Linguistic Learning of Event Semantics

Typologically diverse languages offer systems of lexical and grammatical aspect that allow speakers to focus on facets of event structure in ways that comport with the specific communicative setting and discourse constraints they face. In this paper, we look specifically at captions of images across Arabic, Chinese, Farsi, German, Russian, and Turkish and describe a computational model for predicting lexical aspects. Despite the heterogeneity of these languages, and the salient invocation of distinctive linguistic resources across their caption corpora, speakers of these languages show surprising similarities in the ways they frame image content. We leverage this observation for zero-shot cross-lingual learning and show that lexical aspects can be predicted for a given language despite not having observed any annotated data for this language at all.

==> sections/background.tex <==
\section{Background and Related Work}
\label{sec:methods}

The morphology of Arabic, Farsi, Chinese and Turkish organizes eventualities along different principles. 
While English, Farsi, Arabic and Turkish are predominantly tense languages, Chinese uses particles to add specific aspectual value to the language~\cite{klein2000aspect}. In addition, English, Arabic, Farsi and Turkish differ as to which distinctions are lexicalized in the past \cite{norman1988chinese}.

Tense indicates the temporal location of a situation with respect to salient temporal landmarks; it's deictic. Aspect is not deictic; it offers an intrinsic characterization of the temporal dynamics of a situation. Lexical aspect describes the inherent dynamics of a described eventuality, while grammatical aspect qualifies key features of these dynamics as they contribute to compositional semantics. 

% Chinese has grammatical particles that provide aspect information and can help indicate the temporal flow of events \cite{yang2014l2}. There are three most frequent aspectual particles in Chinese: Perfective, Experiential and Imperfective \cite{huang1989aspectual,peck2013aspectual}. Alternatively, temporal reference can simply be inferred from the context~\cite{li1989mandarin}. Chinese also has a different notion for sentences from English. A sentence can, and often will, have more than one verb without any conjunction \cite{tiee1986reference}.

On the contrary, Arabic and Farsi are morphologically rich languages. Although there exist exceptions, Arabic has a regular verbal morphological system where verbs inflect for aspect, mood, voice and subject.

The morphological system in Farsi includes several different affixes creating different forms. It has three moods: indicative, subjunctive, imperative; two tenses, past and non-past and five main grammatical aspects: Narrative (\FR{نقلی}
), Presedent (\FR{پیشین})
, imperfect (\FR{استمراری})
, Progressive (\FR{مستمر})
and simple (\FR{ساده}).
Narrative narrates a result from a previous action; precedent refers to a completed action in the past but linked to a later time; imperfect indicates the duration and progressive that expresses an incomplete action in progress at a specific time. 
% refers to an event that was completed before another past action

Farsi verbs are either simple or compound. 
Any lexical unit which contains only a verbal root is a simple verb (e.g. verbal root: \FR{رفتن} ‘to go'). The lexical unit which contain either a prefix plus a verbal root, or a nominal plus either a regular verbal root or an auxiliary verb are compound verbs. Related to this is the phenomenon of incorporation, defined by
\cite{spencer1991morphological} as the situation in which “a word forms a kind of compound with its direct object, or adverbial modifiers while retaining its original syntactic function.” \newcite{baker1998berkeley} has proposed a theory for such cases in which the key operation is the incorporation by the syntactic movement of a lexical head by a lexical category, specifically a verb. 
Noun incorporation is productive in Farsi. \newcite{baker2006linkers} explain that for languages with this property, the noun, as well as tense and aspect, precede the verb, whereas agreement follows the verb. 
%Examples in the appendix. 
The compound verb in is `ground eat-PRS-IPFV-1SG’ where the nominal part is
`ground’ and the imperfective marker before the verbal part represents the tense. The verbal stem is `eat' which is followed by the `first person singular verb ending' representing the agreement.

As for the lexicality of compound verbs, \newcite{baker1985c} employs a conservative approach, stating that perhaps both definitions apply since on the one hand, Farsi complex predicates allow nominalization, and on the other hand, their constituents can be separated. Similar to English, that distinguishes between states and two main type of events, Arabic and Farsi have three main classes of lexical aspect namely state, telic and atelic. Telic events express and action tending towards the goal. Atelic events, however, do not have an endpoint \cite{smith2013parameter}. Stative, telic, and atelic are translated accordingly to:
Saade (\FR{ساده})
, Lahze'e
(\FR{لحظه‌ای})
, and Ista
(\FR{ایستا})
  \cite{aspect}.

% Chinese does not have the grammatical category of tense, because the concept denoted by tense in other languages is indicated by content words like adverbs of time or it is simply implied by context.  For example, the verb for "do" is 
% \begin{CJK}{UTF8}{gbsn}
% 做 (zuo)
% \end{CJK}, which is used to describe all past, present, and future events. Since the verb remains the same, temporal reference is instead indicated by the time expressions~\cite{lin2006time}, for example: 
% \begin{exe}
%     \ex \begin{CJK}{UTF8}{gbsn}昨天\space\space\space\space\space\space\space我做了\space\space\space\space\space批萨。\end{CJK}
%     \\
%     Yesterday I do\space PFV pizza.\\
%     Yesterday I made pizza.
% \end{exe}
% Alternatively, temporal reference can simply be inferred from the context~\cite{li1989mandarin}. However, Chinese has grammatical particles that provide aspectual information and can help indicate the temporal flow of events~\cite{yang2014l2}. There are three most frequent aspectual particles in Chinese~\cite{huang1989aspectual,peck2013aspectual}: Perfective, Experiential and Imperfective, as seen in the following examples:

% \begin{exe}
%     \ex 
%         \begin{CJK}{UTF8}{gbsn}
%             我做\space了\space\space\space\space\space一\space\space\space锅\space\space汤。\\
%             I \space\space do PFV one pot soup.\\
%             I have made a pot of soup.
%         \end{CJK}
%     \ex 
%         \begin{CJK}{UTF8}{gbsn}
%             你\space\space\space做\space\space过\space\space\space\space这件事。\\
%             You do EXP this event.\\
%             You did this before.
%         \end{CJK}
%     \ex 
%         \begin{CJK}{UTF8}{gbsn}
%             他\space\space正\space\space\space做\space着\space\space\space\space\space\space家庭作业。\\
%             He now do IPFV homework.\\
%             He is doing the homework.
%         \end{CJK}        
% \end{exe}

% The three most commonly used particles to indicate such grammatical aspects are 
% \begin{CJK}{UTF8}{gbsn}
% 了(perfective), 过(experiential), 在, 着(Imperfective).
% \end{CJK}
% Perfective and experiential aspects are commonly associated with past events. Perfective aspect. particularly, is used to present the viewpoint of ``an event in its entirety''~\cite{li1989mandarin}. The experiential aspect is referring to the property of having experienced the event~\cite{sun2006chinese}. The crucial difference between perfective and experiential aspect is that the perfective marks the action in the past as having an influence at the time of utterance. Experiential aspect further implies discontinuity~\cite{93322320150101}. Imperfective aspect markers denote ongoing actions or states; they are used to describe a situation where the agent is experiencing the action while the utterance takes place. These grammatical markers modify the meaning of the sentence rather than serving as operators that change the meaning of the sentence.  Therefore, unlike in English, they tend to reinforce lexical aspect rather than modifying it: \newcite{huang2005telicity, huang1989aspectual, peck2013aspectual} report that perfective and experiential descriptions are typically telic; imperfective ones, typically atelic. 

% Chinese has a different notion for sentences from English. A sentence can, and often will, have more than one verb~\cite{tiee1986reference}. In English, only one verb carries the tense and aspect information. The other verbs need to be infinitive, if no conjunction is involved. In Chinese, however, a sentence can have multiple verbs, each being a verb phrase, without any conjunction.
% Chinese has a different notion for sentences from English. A sentence can, and often will, have more than one verb~\cite{tiee1986reference}. In English, only one verb carries the tense and aspect information. The other verbs need to be infinitive, if no conjunction is involved. In Chinese, however, a sentence can have multiple verbs, each being a verb phrase, without any conjunction.

% On the contrary, Arabic and Farsi are morphologically rich languages. Although there exist exceptions, Arabic has a regular verbal morphological system where verbs inflect for aspect, mood, voice and subject.



% On the contrary, Arabic and Farsi are morphologically rich languages. Although there exist exceptions, Arabic has a regular verbal morphological system where verbs inflect for aspect, mood, voice and subject. The verbal subject is specified by three features: person, gender and number. Person has three values: 1st (speaker, \AR {متكلم}),
% 2nd (addressee, \AR{مخاطب}) and 3rd (other, \AR{غائب }), gender has two values: masculine or feminine, and number has three values: singular, dual, and plural. The verbal subject is indicated through affixations, whose form is constrained by verbal aspect and mood. Arabic verbs have three grammatical aspects: perfective (\AR{مضارع}), imperfective (\AR{ماضي}), and imperative (\AR{أمر}). The perfective aspect indicates that actions described are completed as opposed to the imperative aspect which does not specify any such information. Whereas the imperative aspect is the command form of the verb. Arabic has also three common moods which only vary for the imperfective aspect: indicative (\AR{مرفوع}), subjunctive (\AR{منصوب}), and jussive (\AR{مجزوم}). Whereas, the perfective aspect does not vary by mood. It is worth noting that there are no specific morphemes in Arabic corresponding to tense such as past, present, or future. However, the various tense values are expressed through a combination of aspect, mood and supporting particles. Lastly, voice in Arabic can be passive or active and it is only indicated through a change in vocalism \cite{arabic-nlp-intro}.

% The morphological features of Arabic are usually represented by: \textit{Tense} (past, non-past), \textit{Person} (1st, 2nd, 3rd), \textit{Grammatical Aspect} (Perfective, Imperfective), \textit{Number} (Singular, Plural, Dual), \textit{Mood \AR{حالات}} (Indicative \AR{مرفوع}, Subjunctive \AR{منصوب}, Jussive \AR{مجزوم}), \textit{Voice \AR{صيغات}}, \textit{Gender \AR{الجنس}} (Feminine \AR{مؤنث}, Masculine \AR{مذكر}) \cite{arabic-nlp-intro}.
% Grammatical aspects in Arabic are used to express the time flow of actions \cite{aspect-in-arabic-russian}. The imperfective aspect is used to express habits and facts such as 'she is running' or 'she runs every morning'. 
% To mark the verb for person, number and gender, suffixes are added if the verb is perfective. Whereas the imperfective verbs are marked by adding a combination of suffixes and prefixes. The inflections of a verb in Arabic depends on its tense. The root (lemma) of a verb in Arabic represents the past tense. 


% In addition to these purely verbal forms, Arabic makes frequent use of a derived adjective form, the active participle is a number of quasi-verbal functions. 


% The morphological system in Farsi includes several different affixes creating different forms. It has three moods: indicative, subjunctive, imperative; two tenses, past and non-past and five main grammatical aspects: Narrative (\FR{نقلی}
% ), Presedent (\FR{پیشین})
% , imperfect (\FR{استمراری})
% , Progressive (\FR{مستمر})
% and simple (\FR{ساده}).
% Narrative narrates a result from a previous action; precedent refers to a completed action in the past but linked to a later time; imperfect indicates the duration and progressive that expresses an incomplete action in progress at a specific time. 
% % refers to an event that was completed before another past action

% Farsi verbs are either simple or compound. 
% Any lexical unit which contains only a verbal root is a simple verb (e.g. verbal root: \FR{رفتن} ‘to go'). The lexical unit which contain either a prefix plus a verbal root, or a nominal plus either a regular verbal root or an auxiliary verb are compound verbs. Related to this is the phenomenon of incorporation, defined by
% \cite{spencer1991morphological} as the situation in which “a word forms a kind of compound with its direct object, or adverbial modifiers while retaining its original syntactic function.” \newcite{baker1998berkeley} has proposed a theory for such cases in which the key operation is the incorporation by the syntactic movement of a lexical head by a lexical category, specifically a verb. 
% Noun incorporation is productive in Farsi. \newcite{baker2006linkers} explain that for languages with this property, the noun, as well as tense and aspect, precede the verb, whereas agreement follows the verb. Examples in the appendix. 

% Consider the following example:
% \begin{exe}
%     \ex \textrm{ }
% \end{exe}
% \begin{tabular}{rrrrr}
%     \FR{می‌خورم.}
%     &
%     \FR{زمین}
%     &
%     \FR{اینجا}
%     &
%     \FR{همیشه}
%     &
%     \FR{من}
%     \\
%     eat-\small{PRS-IPFV-1SG}
%     &
%     ground
%     &
%     here
%     &
%     always
%     &
%     I
%     \\
%     \multicolumn{5}{r}{I always fall here.}
% \end{tabular}\\

% The compound verb in is `ground eat-PRS-IPFV-1SG’ where the nominal part is
% `ground’ and the imperfective marker before the verbal part represents the tense. The verbal stem is `eat' which is followed by the `first person singular verb ending' representing the agreement.

% As for the lexicality of compound verbs, \newcite{baker1985c} employs a conservative approach, stating that perhaps both definitions apply since on the one hand, Farsi complex predicates allow nominalization, and on the other hand, their constituents can be separated. Similar to English, that distinguishes between states and two main type of events, Arabic and Farsi have three main classes of Aktionsart namely state, telic and atelic. Telic events express and action tending towards the goal. Atelic events, however, do not have an endpoint \cite{smith2013parameter}.


Stative, telic, and atelic are translated accordingly to:
Saade (\FR{ساده})
, Lahze'e
(\FR{لحظه‌ای})
, and Ista
(\FR{ایستا})
  \cite{aspect}. Example (6) is a Farsi sentences describing an Ista event. Example (7), (8) are two Arabic examples with telic and stative lexical aspects.
 
%  Example (6) and (7) are two Farsi sentences with Lahzei and Ista events. Example (8), (9) and (10) 
%  are three Arabic sentences with different lexical aspects.
 
% \begin{exe}
% \ex \textrm{ }
% \end{exe}
% \begin{flushright}
% \begin{tabular}{rrrr}
%     \FR{تقسیم}
%     &
%     \FR{را}
%     &
%     \FR{کیک} 
%     &
%     \FR{مردی}
%     \\
%     slice
%     & 
%     \small{CONJ}
%     & 
%     cake
%     &
%     \small{ART}-Man
% \end{tabular}
% \begin{tabular}{r}
%     \FR{می‌کند.}
%      \\
%      do-\small{PRS-IPFV-3SG}
%      \\ 
%      A man is slicing the cake.
% \end{tabular}
% \end{flushright}

\begin{exe}
    \ex \textrm{ }
\end{exe}
\begin{flushright}
\begin{tabular}{rrrrrr}
    \FR{تنیس}
    &
    \FR{زن}
    &
    \FR{یک}
    &
    \FR{و}
    &
    \FR{مرد} 
    &
    \FR{یک}
    \\
    tennis
    &
    woman
    & 
    one
    & 
    and
    & 
    man
    & 
    One
\end{tabular}

\begin{tabular}{rr}
    \FR{می‌کنند.}
    &
    \FR{بازی}
    \\
    do-\small{PRS-IPFV-3PL}
    &
    play
\end{tabular}

A man and a woman are playing Tennis.
\end{flushright}

% \begin{exe}
% \ex \textrm{ }
% \end{exe}
% \begin{flushright}
% \begin{tabular}{rrr}
%     \AR{مبكراً}
%     &
%     \AR{الطفل}
%     &
%     \AR{ينام}
%     \\
%     early
%     & 
%     baby
%     & 
%     sleep-PRS-MASC-IPFV-3G 

% \end{tabular}
% The baby sleeps early.
% \end{flushright}

\begin{exe}
\ex \textrm{ }
\end{exe}
\begin{flushright}
\begin{tabular}{rrrr}
    \AR{التفاحة}
    &
    \AR{الفتاة}
    &
    \AR{أكلت}
    \\
    apple
    & 
    girl
    & 
    ate-PST-FEM-PFV-3SG
\end{tabular}
The girl ate the apple.
\end{flushright}

\begin{exe}
\ex \textrm{ }
\end{exe}
\begin{flushright}
\begin{tabular}{rrr}
    \AR{جميلاً}
    &
    \AR{الجبل}
    &
    \AR{كان}
    \\
    beautiful
    & 
    mountain
    &      
    was-PST-MASC-PFV-3SG
\end{tabular}
The mountain was beautiful.
\end{flushright}
% Aktionsart in Arabic represent whether the event evoked by the verbs constellations
% has a natural endpoint.
% Events that describe a condition rather than activities are \textit{stative}. Events that describe an achievement or mark a natural endpoint that are mostly perfective are \textit{telic} and events that describe an ongoing event are \textit{atelic}.


% \begin{exe}
% \ex \textrm{ }
% \end{exe}
% \begin{flushright}
% \begin{tabular}{rrr}
%     \AR{مبكراً}
%     &
%     \AR{الطفل}
%     &
%     \AR{ينام}
%     \\
%     early
%     & 
%     baby
%     & 
%     sleep-PRS-MASC-IPFV-3G 

% \end{tabular}
% The baby sleeps early.
% \end{flushright}

% \begin{exe}
% \ex \textrm{ }
% \end{exe}
% \begin{flushright}
% \begin{tabular}{rrrr}
%     \AR{التفاحة}
%     &
%     \AR{الفتاة}
%     &
%     \AR{أكلت}
%     \\
%     apple
%     & 
%     girl
%     & 
%     ate-PST-FEM-PFV-3SG
% \end{tabular}
% The girl ate the apple.
% \end{flushright}

% \begin{exe}
% \ex \textrm{ }
% \end{exe}
% \begin{flushright}
% \begin{tabular}{rrr}
%     \AR{جميلاً}
%     &
%     \AR{الجبل}
%     &
%     \AR{كان}
%     \\
%     beautiful
%     & 
%     mountain
%     &      
%     was-PST-MASC-PFV-3SG
% \end{tabular}
% The mountain was beautiful.
% \end{flushright}

% \begin{exe}
    
% 	\ex \AR{ينام الطفل مبكراً} (\textit{atelic}) \\
% 	    early baby sleep-PRS-MASC-IPFV-3G  \\
% 	    The baby sleeps early
% 	\ex \AR{أكلت الفتاة التفاحة} (\textit{telic}) \\
% 	    apple girl ate-PST-FEM-PFV-3SG\\
% 	    The girl ate the apple
% 	\ex \AR{كان الجبل جميلاً} (\textit{stative}) \\
% 	    beautiful mountain was-PST-MASC-PFV-3SG\\
% 	    The mountain was beautiful
% \end{exe}

% \paragraph{Arabic.} 



% Arabic represents a prime example of diglossia \cite{ferguson}, where the formal language which is used in written communication is significantly different from the informal language and verbal communication. 
% %
% The morphological features of Arabic are usually represented by: \textit{Person} (1st, 2nd, 3rd), \textit{Grammatical Aspect} (Perfective, Imperfective), \textit{Number} (Singular, Plural, Dual), \textit{Mood \AR{حالات}} (Indicative \AR{مرفوع}, Subjunctive \AR{منصوب}, Jussive \AR{مجزوم}), \textit{Voice \AR{صيغات}} (Passive \AR{مجهول}, Active \AR{معلوم}), \textit{Gender \AR{الجنس}} (Feminine \AR{مؤنث}, Masculine \AR{مذكر}), \textit{State} (Indefinite, Definite, Construct), and \textit{Case} (Nominative, Accusative, Genitive) \cite{arabic-nlp-intro}.\\
% % The grammatical aspect of a conjugated verb in Arabic is usually marked as Perfective, if the conjugation appears as a \textit{suffix}. Whereas it is marked as Imperfective, if the conjugation appear as \textit{suffixes} and \textit{prefixes}.
% The grammatical aspects of verbs in Arabic correspond to a distinction between past tense and non-past tense. The perfective aspect is used to describe verbs in the past tense and it expresses events such as  'she did' as opposed to 'she was doing'. Whereas the imperfective aspect is used to describe continuous verbs or to express habits and facts such as 'she is running' or 'she runs every morning'. To mark the verb for person, number and gender, suffixes are added if the verb is perfective. Whereas the imperfective verbs are marked by adding a combination of suffixes and prefixes.
% % In addition to these purely verbal forms, Arabic makes frequent use of a derived adjective form, the active participle is a number of quasi-verbal functions. 

% Aktionsart in Arabic represent whether the event evoked by the verbs constellations
% has a natural endpoint.
% Events that describe a condition rather than activities are \textit{stative}. Events that describe an achievement or mark a natural endpoint that are mostly perfective are \textit{telic} and events that describe an ongoing event are \textit{atelic}.


% \begin{exe}
    
% 	\ex \AR{ينام الطفل مبكراً} (\textit{atelic}) \\
% 	    early baby sleep-PRS-MASC-IPFV-3G  \\
% 	    The baby sleeps early
% 	\ex \AR{أكلت الفتاة التفاحة} (\textit{telic}) \\
% 	    apple girl ate-PST-FEM-PFV-3SG\\
% 	    The girl ate the apple
% 	\ex \AR{كان الجبل جميلاً} (\textit{stative}) \\
% 	    beautiful mountain was-PST-MASC-PFV-3SG\\
% 	    The mountain was beautiful
% \end{exe}



% \paragraph{Chinese.} 

% Chinese has a different notion for sentences from English. A sentence can, and often will, have more than one verbs~\cite{tiee1986reference}.  In English, only one verb carries the tense and aspect information. The other verbs need to be infinitive, if no conjunction is involved. In Chinese, however, a sentence can have multiple verbs, each being a verb phrase, without any conjunction.


% Chinese does not use verb conjugations, or any other forms of grammatical markers, to indicate tense. For example, the verb for "do" is 
% \begin{CJK}{UTF8}{gbsn}
% 做 (zuo)
% \end{CJK}, which is used for the past, present, and future tenses. As much as the verb remains the same, the tense is instead indicated by the expression of time~\cite{lin2006time}, for example: 
% \begin{exe}
%     \ex \begin{CJK}{UTF8}{gbsn}昨天我做了批萨。\end{CJK}
%     \\
%     Yesterday I do PFV pizza.\\
%     Yesterday I made pizza.
% \end{exe}

% Sometimes the tense can also simply be inferred from the context~\cite{li1989mandarin}.

% However, Chinese needs grammatical markers to indicate aspects. Aspect markers in Chinese are used to indicate the temporal flow of events~\cite{yang2014l2}. There are three most common grammatical aspects in Chinese~\cite{huang1989aspectual,peck2013aspectual}: Perfective, Experiential and Imperfective. The following examples present three sentences with these aspects accordingly:


% \begin{exe}
%     \ex 
%         \begin{CJK}{UTF8}{gbsn}
%             我做了一锅汤。\\
%             I do PFV one pot soup.\\
%             I have made a pot of soup.
%         \end{CJK}
%     \ex 
%         \begin{CJK}{UTF8}{gbsn}
%             你做过这件事。\\
%             You do EXP this event.\\
%             You did this before.
%         \end{CJK}
%     \ex 
%         \begin{CJK}{UTF8}{gbsn}
%             他正做着家庭作业。\\
%             He now do IPFV homework.\\
%             He is doing the homework.
%         \end{CJK}        
% \end{exe}

% The three most commonly used particles to indicate such grammatical aspects are 
% \begin{CJK}{UTF8}{gbsn}
% 了(perfective), 过(experiential), 在, 着(Imperfective)
% \end{CJK}
% . Perfective and experiential aspects are commonly associated with past events. Perfective aspect particularly, is used to present the viewpoint of "an event in its entirety"~\cite{li1989mandarin}. The experiential aspect is referring to the property of having experienced the event~\cite{sun2006chinese}. The crucial difference between perfective and experiential aspect is whether the action in the past has an influence at the time of utterance. Imperfective aspect markers denote ongoing actions or states. 



% Perfective and experiential aspects are meant to describe events that happened in the past with a definite endpoint, regardless of the current influence. Imperfective is used to describe a situation where the agent is experiencing the action while the utterance takes place. \newcite{huang2005telicity, huang1989aspectual, peck2013aspectual} consider perfective and experiential descriptions mostly as telic and the imperfective descriptions as atelic event. 


% \textbf{Farsi.} The morphological system in Farsi includes several different affixes creating different forms. It has three moods: indicative, subjunctive, imperative; two tenses, past and non-past and five main grammatical aspects: Narrative (\FR{نقلی}
% ), Presedent (\FR{پیشین})
% , imperfect (\FR{استمراری})
% , Progressive (\FR{مستمر})
% and simple (\FR{ساده}).
% Narrative narrates a state resulting from a previous action; precedent refers to an event that was completed before another past action;  imperfect indicates the duration and progressive that expresses an incomplete action in progress at a specific time. 

% Verbal phrases are divided into simple and compound. 
% Any verbal phrase which contains only a verbal root is a simple verb (e.g. verbal root: \FR{رفتن} ‘to go'. The verbal phrases which contain either a prefix plus a verbal root, or a nominal plus either a regular verbal root or an auxiliary verb are compound verbs. Related to this is the phenomenon of incorporation, defined by
% \cite{spencer1991morphological} as the situation in which “a word forms a kind of compound with its direct object, or adverbial modifiers while retaining its original syntactic function.” \newcite{baker1998berkeley} has proposed a theory for such cases in which the key operation is the incorporation by the syntactic movement of a lexical head by a lexical category, specifically a verb. 
% Noun incorporation is productive in Farsi. \newcite{baker2006linkers} explain that for languages with this property, the noun, as well as tense and aspect, precede the verb, whereas agreement follows the verb.  Consider the following example:
% \begin{exe}
%     \ex \textrm{ }
% \end{exe}
% \begin{tabular}{rrrrr}
%     \FR{می‌خورم.}
%     &
%     \FR{زمین}
%     &
%     \FR{اینجا}
%     &
%     \FR{همیشه}
%     &
%     \FR{من}
%     \\
%     eat-\small{PRS-IPFV-1SG}
%     &
%     ground
%     &
%     here
%     &
%     always
%     &
%     I
%     \\
%     \multicolumn{5}{r}{I always fall here.}
% \end{tabular}\\

% The compound verb in is `ground eat-PRS-IPFV-1SG’ where the nominal part is
% `ground’ and the imperfective marker before the verbal part represents the tense. The verbal stem is `eat' which is followed by the `first person singular verb ending' representing the agreement.

% As for the lexicality of compound verbs, \newcite{baker1985c} employs a conservative approach, stating that perhaps both definitions apply since on the one hand, Farsi complex predicates allow nominalization, and on the other hand, their constituents can be separated. 

% The lexical aspect of verbs marks the manner of their progression. It refers to both the verb phrase and the root. Farsi has three classes of lexical aspect:
% Saade (\FR{ساده})
% , Lahze'e
% (\FR{لحظه‌ای})
% , and Ista
% (\FR{ایستا})
% that can be mapped accordingly to stative, telic and atelic. Lahze'e and Ista distinguish between two different classes of events. Lahzei refers to events that are complete whereas Ista references to incomplete actions \cite{aspect,smith2013parameter}. The followings are two examples of Lahzei and Ista events.
% \begin{exe}
% \ex \textrm{ }
% \end{exe}
% \begin{flushright}
% \begin{tabular}{rrrr}
%     \FR{تقسیم}
%     &
%     \FR{را}
%     &
%     \FR{کیک} 
%     &
%     \FR{مردی}
%     \\
%     slice
%     & 
%     \small{CONJ}
%     & 
%     cake
%     &
%     \small{ART}-Man
% \end{tabular}
% \begin{tabular}{r}
%     \FR{می‌کند.}
%      \\
%      do-\small{PRS-IPFV-3SG}
%      \\ 
%      A man is slicing the cake.
% \end{tabular}
% \end{flushright}

% \begin{exe}
%     \ex \textrm{ }
% \end{exe}
% \begin{flushright}
% \begin{tabular}{rrrrrr}
%     \FR{تنیس}
%     &
%     \FR{زن}
%     &
%     \FR{یک}
%     &
%     \FR{و}
%     &
%     \FR{مرد} 
%     &
%     \FR{یک}
%     \\
%     tennis
%     &
%     woman
%     & 
%     one
%     & 
%     and
%     & 
%     man
%     & 
%     One
% \end{tabular}

% \begin{tabular}{rr}
%     \FR{می‌کنند.}
%     &
%     \FR{بازی}
%     \\
%     do-\small{PRS-IPFV-3PL}
%     &
%     play
% \end{tabular}

% A man and a woman are playing Tennis.
% \end{flushright}



==> todo.tex <==
--add the COLING work after it's accepted

--
